Neural Network-Based Abstract Generation for Opinions and Arguments

We study the problem of generating abstractive summaries for opinionated text. We propose an attention-based neural network model that is able to absorb information from multiple text units to construct informative, concise, and fluent summaries. An importance-based sampling method is designed to allow the encoder to integrate information from an important subset of input. Automatic evaluation indicates that our system outperforms state-of-the-art abstractive and extractive summarization systems on two newly collected datasets of movie reviews and arguments. Our system summaries are also rated as more informative and grammatical in human evaluation.

==> scoring.tex <==
%We first introduce an importance estimation model. 
% the general description on what does the model do
We now described importance estimation model, which outputs importance scores for text units, used in Section~\ref{mul_inputs}.

Given a pair of text units $x^1,...,x^{M}$ and their summary $y$. We compute the number of overlapping content words between each text unit and its associated summary as its gold-standard importance score. The scores are normalized to $[0,1]$.

Each text unit $x^k$ is represented as an $d-$dimensional feature vector {\small $\mathbf{\mathbf{r_{k}}}\in \mathbb{R}^{d}$}, with label {\small $l_{k}$}. 
%For simplicity, we use $\mathbf{r}$ to represent a text unit and $l$ to be its label wherever there is no ambiguity. 
Text units in the training data are denoted with a feature matrix {\small $\mathbf{\tilde{R}}$} with a label vector {\small $\mathbf{\tilde{L}}$}. We learn {\small $f(x^{k})=\mathbf{r_{k}}\cdot \mathbf{w}$} by minimizing 
%
{\small $||\mathbf{\tilde{R}} \mathbf{w} - \mathbf{\tilde{L}}||_{2}^{2} + \beta \cdot ||\mathbf{w}||_{2}^{2}$}. 
%
Features are listed in Table~\ref{tab:features_importance}.  
%
Pairwise preference constraints have been utilized for learning ranking models~\cite{Joachims:2002:OSE:775047.775067}. We thus consider {\it pairwise preference-based regularizing constraint} to incorporate a bias toward summary-worthy text unit: \\
%
%{\small $\lambda\cdot \sum_{c_{i}}\sum_{l_{c_{i}, j} > 0, l_{c_{i}, k} =0} ||(\mathbf{r_{c_{i}, j}}-\mathbf{r_{c_{i}, k}})\cdot \mathbf{w}- 1||_{2}^{2}$}
%
%where $c_{i}$ is a cluster of text units to be summarized. 
%Term {\small $(\mathbf{r_{c_{i}, j}}-\mathbf{r_{c_{i}, k}})\cdot \mathbf{w}$} enforces the separation of summary-worthy text from the others.
{\small $\lambda\cdot \sum_{\mathcal{T}} \sum_{x^{p}, x^{q}\in \mathcal{T}, l_{p} > 0, l_{q} =0} ||(\mathbf{r_{p}}-\mathbf{r_{q}})\cdot \mathbf{w}- 1||_{2}^{2}$}
%
where $\mathcal{T}$ is a cluster of text units to be summarized. 
Term {\small $(\mathbf{r_{p}}-\mathbf{r_{q}})\cdot \mathbf{w}$} enforces the separation of summary-worthy text from the others. 
We further construct {\small$\mathbf{\tilde{R}^{\prime}}$} to contain all the pairwise differences {\small$(\mathbf{r_{p}}-\mathbf{r_{q}})$}. {\small$\mathbf{\tilde{L}^{\prime}}$} is a vector of same size as {\small$\mathbf{\tilde{R}^{\prime}}$} with each element as $1$. Thus, the objective function to minimize is:


{\small
\begin{equation}
J(\mathbf{w})=||\mathbf{\tilde{R}} \mathbf{w} - \mathbf{\tilde{L}}||_{2}^{2} + \lambda\cdot ||\mathbf{\tilde{R}^{\prime}} \mathbf{w} - \mathbf{\tilde{L}^{\prime}}||_{2}^{2}+\beta\cdot ||\mathbf{w}||_{2}^{2}
\end{equation}
}

With $\tilde{\boldsymbol \beta}=\beta \cdot \mathbf{I_{d}}$ and $\tilde{\boldsymbol \lambda} = \lambda \cdot \mathbf{I_{|R^{\prime}|}}$, then the \textbf{closed-form} solution for $\hat{\mathbf{w}}$ is:

{\small
\begin{equation}
\hat{\mathbf{w}}=(\mathbf{\tilde{R}^{T}\tilde{R}+\tilde{R}^{\prime T} \tilde{\boldsymbol \lambda} \tilde{R}^{\prime}}+\tilde{\boldsymbol \beta})^{-1}(\mathbf{\tilde{R}^{T}\tilde{L}+\tilde{R}^{\prime T} \tilde{\boldsymbol \lambda} \tilde{L}^{\prime}})
\end{equation}
}

\begin{table}[htbp]
\centering
    {\fontsize{9}{10}\selectfont
    \setlength{\baselineskip}{0pt}
    \setlength{\tabcolsep}{0.8mm}
    \begin{tabular}{|l|l|}
    \hline

	- num of words & - category in General Inquirer\\
	- unigram & ~\cite{stone66}\\
	- num of POS tags & - num of positive/negative/neutral \\ 
	- num of named entities & ~ words (General Inquirer,\\
	- centroidness~\cite{Radev01experimentsin} & ~MPQA~\cite{Wilson:2005:RCP})\\
	- avg/max TF-IDF scores & \\ 
	\hline
	\end{tabular}
	}
    \caption{Features used for importance estimation.} 
	\label{tab:features_importance}
\end{table}
